When Federated Learning Meets Pre-trained Language Models' Parameter-Efficient Tuning Methods

With increasing privacy concerns on data, recent studies have made significant progress using federated learning (FL) on privacy-sensitive natural language processing (NLP) tasks. Much literature suggests fully fine-tuning pre-trained language models (PLMs) in the FL paradigm can mitigate the data heterogeneity problem and close the performance gap with centralized training. However, large PLMs bring the curse of prohibitive communication overhead and local model adaptation costs for the FL system. To this end, we introduce various parameter-efficient tuning (PETuning) methods into federated learning. Specifically, we provide a holistic empirical study of representative PLMs tuning methods in FL. The experimental results cover the analysis of data heterogeneity levels, data scales, and different FL scenarios. Overall communication overhead can be significantly reduced by locally tuning and globally aggregating lightweight model parameters while maintaining acceptable performance in various FL settings. To facilitate the research of PETuning in FL, we also develop a federated tuning framework FedPETuning, which allows practitioners to exploit different PETuning methods under the FL training paradigm conveniently. The source code is available at \url{https://github.com/iezhuozhuo/FedETuning/tree/deltaTuning}.

==> Old_4_Experiment.tex <==
In this section, we conduct extensive experiments to investigate the performance of four representative PETuning methods under the FL setting. To be more concrete, 

% we aim to answer the following questions:

\begin{itemize}
  % \item  Can we achieve a better balance between communication cost and model performance with the PETuning methods than fine-tuning?
  \item  \textbf{RQ1}: How effective are PETuning methods for reducing resource costs (i.e., communication overhead and local model adaptation cost) in the FL system? (see Section \ref{rq:resouce_cost})
  
  \item  \textbf{RQ2}: How do the PETuning methods compare to full fine-tuning in terms of performance under the FL setting? (see Section \ref{rq:acc})

  \item  \textbf{RQ3}: What is the impact of local client's data scale on all tuning methods? (see Section \ref{rq:data_scale})

  % \item \textbf{RQ4}: What is the impact of increasing local epochs on PETuning methods under the federated training paradigm? (see Section \ref{rq4:epoches})
  
  \item  \textbf{RQ4}: What is the impact of different levels of data Non-IID on the PETuning method? (see Section \ref{rq:alpha})

  \item \textbf{RQ5}: What is the impact of different FL scenarios on PETuning methods? (see Section \ref{rq:fl_scen})
\end{itemize}

% we first introduce a new FL benchmark \fedglue, which is derived from the vanilla GLUE and complies with the general FL data partitioning method. Secondly, we perform holistic comparisons among four representative PETuning methods on \fedglue, including the utility and communication overhead analyses.

% (3) furthermore, we probe the privacy-preserving capability and robustness of various PETuning methods in the conventional FL scenario and examine how effects on performance after inserting defense measures.

\begin{table}[]
\centering
\small
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Task} & \textbf{\# Train} & \textbf{\# Dev.} & \textbf{\# Test} & \textbf{Metric}  \\ \midrule
RTE       & 2,241 &  249 &  277  & Accuracy \\
MRPC      & 3,301 &  367 &  408  & F1 Score \\ 
% CoLA      & 7695 &  856 &  1043  & matthews \\
SST-2     & 66,675 &  674 &  872  & Accuracy \\
QNLI      & 103,695 &  1,048 &  5,463 & Accuracy \\
QQP       & 360,210 &  3,639 &  40,430 & Accuracy \\ 
MNLI   & 388,774 &  3,928 &  9,815 & Accuracy \\
\bottomrule
\end{tabular}
\caption{Dataset descriptions and statistics.}\label{tab:benchmark}
\vspace{-0.4cm}
\end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, scale=0.28]{images/fedgluev1x.pdf}
% \caption{Probability density function of client data distribution. We use the pairwise Jensen–Shannon distance of the label distribution between two clients.} 
% \label{fig:fedgluev1} 
% \vspace{-0.4cm}
% \end{figure}
\subsection{Experiments Setup}
% \subsection{\fedglue}
\subsubsection{Dataset and Non-IID partitioning} 
Our experiments use six datasets from the GLUE benchmark to construct a new FL benchmark called \fedglue for short. The reasons are as follows: (1) Datasets in GLUE  are the \textit{de facto} standard benchmarks for verifying PLMs' effectiveness in natural language understanding, (2) they are heavily used to validate different PETuning methods~\cite{li-liang-2021-prefix,DBLP:journals/corr/abs-2110-07602,zaken2021bitfit,houlsby2019parameter}, and (3) these datasets are large enough and convenient for FL data partitioning (Non-IID). Due to the limitation of the unpublished test set in GLUE, for \fedglue, we follow the previous studies~\cite{liu2022no,zhao2022reduce} and use the original validation set as the new test set and split a part of the training set as the validation set. The data breakdown for this benchmark is in Table~\ref{tab:benchmark}.

For the Non-IID data partitioning, we follow \citet{lin2021fednlp} and partition the datasets by using the Dirichlet distribution as the class priors. In particular, we sample $\mathcal{D} \sim Dir(\alpha)$ and allocate data $\mathcal{D}_k$ to $k$-th client. $\alpha$ determines the degree of Non-IID, and a smaller $\alpha$ generates a high label distribution shift. Unless otherwise mentioned, we set the Dirichlet parameter $\alpha$ = 1.0 as default throughout our experiment. 


% Figure~\ref{fig:fedgluev1} shows the Probability Density Function (PDF) of data distribution among clients.  

% Due to the limitation of the unpublished test set, existing FL studies~\cite{liu2022no,zhao2022reduce} utilize GLUE report performance on the validation set. In their experiment, they train PLMs using the FL paradigm and record the aggregation model's performance result on the validation set after each communication round, ultimately reporting the best validation set performance results. However, their reported results are incomparable, inappropriate, and unveracious to some extent. Since selecting the best model and reporting the best performance on the same dataset,  the model can fall into overfitting in a breeze and beget spuriously high performance~\cite{chen2022revisiting}. On the other hand, the current work uses different partition strategies to simulate the Non-IID data distribution of the FL setting, which makes the reported results not comparable.

% For the sake of more robust and accurate comparisons of different PLMs tuning methods in the FL setting, we reelect six datasets from GLUE to construct a new FL benchmark called \fedglue for short. We chose these six datasets because they are large enough to be partitioned to as many clients as possible. And these datasets, which are classification tasks, are more convenient for the Non-IID data partition. In \fedglue, we use the original validation set as the new test set and split a part of the training set as the validation set. The data breakdown for this benchmark is in Table~\ref{tab:benchmark}.  We set $\alpha$ = 1.0 as default throughout our experiment. Figure~\ref{fig:fedgluev1} shows the Probability Density Function (PDF) data distribution among clients.   

% \footnote{If not specifically mentioned, CS/SC/LC settings correspond to having 10/100/1000 clients at total.}
% In order to evaluate fine-tuning and PETuning methods in a practical FL setting, we consider the Non-IID data partitioning with multiple scales, including cross-silo (CS), standard cross-device (SC), and large-scale cross-device (LC). Following ~\citet{lin2021fednlp} setup, we partition the datasets using the Dirichlet distribution as the class priors wherein the Dirichlet parameter $\alpha$ determines the degree of Non-IID. Concretely, we select \{BoolQ, SST-2, QNLI\} under the CS setting and \{RTE, MRPC, WiC, CoLA\} under the SC setting, and \{QQP, MNLI\} under LC setting. 

% rte: 2241/249/277
% mrpc: 3301/367/408
% cola: 7695/856/1043
% sst-2: 66675/674/872
% qnli: 103695/1048/5463
% qqp: 360210/3639/40430
% mnli: 388774/3928/9815

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% 这是seed=42 %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[ht]
%     \centering
%     \caption{Results of the PETuning Methods on 7 GLUE tasks under full data setting. }
%     % \vspace{-6pt}
%     \scalebox{0.95}{
%     \begin{tabular}{ccccccccc|c}
%     \toprule
%     \multicolumn{2}{c}{Methods}     & RTE & MRPC & CoLA & SST-2 & QNLI & QQP & MNLI & Avg\\

%     % \midrule
%     \midrule
%      \multirow{5}{*}{FedAvg} 
%     & LoRA & 64.3  &  89.4 & 59.0 & \textbf{94.3} & \textbf{90.9} & 87.2 & 85.0 & 81.4 \\
%     & Prefix  & 57.8  &  87.6 & 57.4 & 93.7 & 88.1 & 86.1 & 82.2 & 79.0 \\
%     & Adapter  & \textbf{71.1}  &  90.6 & \textbf{60.8} & 94.0 & 90.7 & 88.6 & \textbf{86.2} & \textbf{83.1} \\
%     & BitFit  & 60.6  &  88.7 & 51.7 & 92.8 & 86.8 & 84.7 & 81.5 &  78.1 \\
%     & Fine-tuning  & 68.6  &  \textbf{91.3} & 60.6 & \textbf{94.3} & 90.7 & \textbf{89.4} & \textbf{86.2} & 83.0 \\
%     \cmidrule{2-10}
%     & Avg &  &   &  &  &  &   &   &  \\
%     \midrule
%     \multirow{5}{*}{Centralized} 
%     & LoRA & 72.9  &  91.1 & 61.6 &  94.6 & \textbf{93.1} & 90.4 & 87.3 & 84.4\\
%     & Prefix  & 70.8  &  91.3 & 60.4 & 94.6 & 91.7 & 89.5 & 86.6 & 83.6 \\
%     & Adapter  & \textbf{76.5}  & 92.0  & \textbf{62.3} &  \textbf{94.8} & 92.9 & 90.9 & \textbf{87.6} & \textbf{85.3} \\
%     & BitFit  & 72.2  &  90.9 & 59.6 & 94.5 & 91.2 & 87.5 & 84.7 &  82.9\\
%     & Fine-tuning  & 74.4  &  \textbf{91.8} & 60.1  & 92.1 & 91.3 & \textbf{91.1} & 85.7 & 83.9\\
%     \cmidrule{2-10}
%     & Avg &  &   &  &  &  &   &   &  \\
%     \bottomrule
%     \end{tabular}  \label{tab:main_results}
%     }
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% 这是5 seeds %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
    \centering
    
    % \scalebox{0.95}{
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccc|lrl}
    \toprule
    Methods  & RTE & MRPC & SST-2 & QNLI & QQP & MNLI & Avg. & \multicolumn{1}{c}{Rel.} & Com. \\
    \midrule
    FedFT  & $\bm{70.3_{1.2}}$ & $\bm{90.7_{0.3}}$ & $\bm{94.0_{0.6}}$ & $\bm{91.0_{0.4}}$  & $\bm{89.5_{0.1}}$ & $\bm{86.4_{0.2}}$ & $\bm{83.1}$ & $100.0$\% & $1$x\\
    FedAP & $69.4_{2.6}$ & $89.1_{1.2}$  &  $93.3_{0.6}$ & $90.9_{0.4}$  & $88.4_{0.2}$ & $86.0_{0.4}$ & $82.4$
     & \yblue{$99.1$\%} & \ygreen{$\uparrow$}$60$x \\
    FedLR & $67.4_{4.2}$ & $84.5_{4.5}$  &  $93.6_{0.5}$ & $90.8_{0.3}$  & $87.4_{0.3}$ & $84.9_{0.4}$ & $81.0$
     & \yblue{$97.5$\%} & \ygreen{$\uparrow$}$141$x \\
    FedPF & $58.6_{2.2}$ & $86.8_{1.0}$ &  $93.0_{0.6}$ & $87.6_{0.5}$  & $85.7_{0.3}$ & $82.2_{0.3}$ & $78.4$
     & $94.3$\% & \ygreen{$\uparrow$}$12$x \\
    FedBF & $61.4_{1.7}$ & $84.6_{2.7}$ &  $92.5_{0.7}$ &  $87.2_{0.5}$ & $84.5_{0.5}$ & $81.7_{0.2}$ & $77.8$ 
     & $93.6$\% & \ygreen{$\uparrow$}$190$x \\

    % \cmidrule{2-8}
    \midrule
    Avg. / Rel. & $65.4$ / $90.8$\% & $87.1$ / \yblue{$95.7$\%} & $93.3$ / \yblue{$99.6$\%} & $89.5$ / \yblue{$97.5$\%} & $87.1$ / \yblue{$96.9$\%} & $84.3$ / \yblue{$97.6$\%} & \multicolumn{3}{c}{-}  \\
    \midrule
    CenFT  & $73.0_{1.4}$ & $90.9_{0.6}$ &  $92.1_{0.5}$ & $90.8_{0.5}$ & $\bm{91.1_{0.2}}$ & $86.0_{0.2}$ & $83.6$ & $100.0$\% & \multicolumn{1}{c}{-} \\
    CenAP & $\bm{76.0_{1.8}}$  & $90.6_{0.8}$ &  $\bm{94.6_{0.5}}$ & $\bm{92.9_{0.1}}$ & $\bm{91.1_{0.1}}$ & $\bm{87.5_{0.2}}$ & $\bm{84.7}$
     & \yred{$101.3$\%} & \multicolumn{1}{c}{-} \\
    CenLR & $74.4_{2.4}$  & $\bm{91.7_{0.6}}$  & $94.0_{0.4}$ & $92.7_{0.6}$ & $90.1_{0.3}$ & $87.0_{0.2}$ & $84.4$ 
     & \yred{$100.9$\%} & \multicolumn{1}{c}{-} \\
    CenPF & $65.6_{5.1}$  & $90.2_{0.9}$  &  $93.7_{0.8}$ & $91.5_{0.2}$ & $89.5_{0.1}$ & $86.7_{0.2}$ & $82.2$ 
     & \yblue{$98.3$\%} & \multicolumn{1}{c}{-} \\
    CenBF  & $70.9_{1.0}$  & $91.3_{0.8}$  &  $94.1_{0.3}$ & $91.3_{0.2}$ & $87.4_{0.2}$ & $84.6_{0.1}$ & $82.6$
     & \yblue{$98.8$\%} & \multicolumn{1}{c}{-} \\
    % \cmidrule{2-8}
    \midrule
     Avg. & $72.0$ & $91.0$ & $93.7$ & $91.8$ & $89.9$ & $86.4$ & \multicolumn{3}{c}{-}  \\
    \bottomrule
    \end{tabular}
}
    \caption{
    Performance results of the PETuning methods on \fedglue under the federated (upper half) and the centralized (bottom half) settings. We show the relative accuracy of PETuning methods to fine-tuning. The difference in communication budget between PETuning methods and fine-tuning is indicated by \ygreen{$\uparrow$}. All experiments are run 5 times with different seeds.
    }\label{tab:main_results}
\end{table*}

%%%%%%%%%%%% 备份 %%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[ht]
%     \centering
    
%     % \scalebox{0.95}{
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{lcccccc|lrl}
%     \toprule
%     Methods     & RTE & MRPC & SST-2 & QNLI & QQP & MNLI & \multicolumn{3}{c}{Avg}\\

%     % \midrule
%     \midrule
%      FedBF & $61.4_{1.7}$ & $84.6_{2.7}$ &  $92.5_{0.7}$ &  $87.2_{0.5}$ & $84.5_{0.5}$ & $81.7_{0.2}$ & $77.8$ 
%      & ($-6.4\%$\yblue{$\downarrow$} & $190$x\yred{$\uparrow$})\\
%      FedPF & $58.6_{2.2}$ & $86.8_{1.0}$ &  $93.0_{0.6}$ & $87.6_{0.5}$  & $85.7_{0.3}$ & $82.2_{0.3}$ & $78.4$
%      & ($-5.7\%$\yblue{$\downarrow$} & $12$x\yred{$\uparrow$})\\
%      FedLR & $67.4_{4.2}$ & $84.5_{4.5}$  &  $93.6_{0.5}$ & $90.8_{0.3}$  & $87.4_{0.3}$ & $84.9_{0.4}$ & $81.0$
%      & ($-2.5\%$\yblue{$\downarrow$} & $141$x\yred{$\uparrow$})\\
%      FedAP & $69.4_{2.6}$ & $89.1_{1.2}$  &  $93.3_{0.6}$ & $90.9_{0.4}$  & $88.4_{0.2}$ & $86.0_{0.4}$ & $82.4$
%      & ($-0.8\%$\yblue{$\downarrow$} & $60$x\yred{$\uparrow$})\\
%      FedFT  & $\bm{70.3_{1.2}}$ & $\bm{90.7_{0.3}}$ & $\bm{94.0_{0.6}}$ & $\bm{91.0_{0.4}}$  & $\bm{89.5_{0.1}}$ & $\bm{86.4_{0.2}}$ & \multicolumn{3}{l}{$\bm{83.1}$}\\
%     % \cmidrule{2-8}
%     \midrule
%      Avg & $65.4$ ($-9.2\%$\ygreen{$\downarrow$}) & $87.1$ ($-4.3\%$\ygreen{$\downarrow$}) & $93.3$ ($-0.4\%$\ygreen{$\downarrow$}) & $89.5$ ($-2.5\%$\ygreen{$\downarrow$}) & $87.1$ ($-3.1\%$\ygreen{$\downarrow$}) & $84.3$ ($-2.4\%$\ygreen{$\downarrow$}) & \multicolumn{3}{c}{-}  \\
%     \midrule
%      BitFit  & $70.9_{1.0}$  & $91.3_{0.8}$  &  $94.1_{0.3}$ & $91.3_{0.2}$ & $87.4_{0.2}$ & $84.6_{0.1}$ & $82.6$
%      & \multicolumn{2}{c}{($-1.2\%$\yblue{$\downarrow$})} \\
%      Prefix & $65.6_{5.1}$  & $90.2_{0.9}$  &  $93.7_{0.8}$ & $91.5_{0.2}$ & $89.5_{0.1}$ & $86.7_{0.2}$ & $82.2$
%      & \multicolumn{2}{c}{($-1.7\%$\yblue{$\downarrow$})} \\
%      LoRA & $74.4_{2.4}$  & $\bm{91.7_{0.6}}$  & $94.0_{0.4}$ & $92.7_{0.6}$ & $90.1_{0.3}$ & $87.0_{0.2}$ & $84.4$ 
%      & \multicolumn{2}{c}{($+1.0\%$\yblue{$\uparrow$})} \\
%      Adapter & $\bm{76.0_{1.8}}$  & $90.6_{0.8}$ &  $\bm{94.6_{0.5}}$ & $\bm{92.9_{0.1}}$ & $\bm{91.1_{0.1}}$ & $\bm{87.5_{0.2}}$ & $\bm{84.7}$
%      & \multicolumn{2}{c}{($+1.3\%$\yblue{$\downarrow$})} \\
%      Fine-tuning  & $73.0_{1.4}$ & $90.9_{0.6}$ &  $92.1_{0.5}$ & $90.8_{0.5}$ & $\bm{91.1_{0.2}}$ & $86.0_{0.2}$ & \multicolumn{3}{l}{$83.6$}\\
%     % \cmidrule{2-8}
%     \midrule
%      Avg & $72.0$ & $91.0$ & $93.7$ & $91.8$ & $89.9$ & $86.4$ & \multicolumn{3}{c}{-}  \\
%     \bottomrule
%     \end{tabular}
% }
%     \caption{Results of the PETuning Methods on 7 GLUE tasks under Non-IID setting.}  \label{tab:main_results}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% 上面是5 seeds %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{table}[]
% \centering
% \small
% \label{tab:communication_exp}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lSS}
% \toprule
% \textbf{Method} & \textbf{\# Trainable Parameters (MB)} & \textbf{Reduction (x)} \\ \midrule
% BitFit   &  2.7   & 178 \\
% Prefix   &  41.2  &   12 \\
% LoRA     &  3.6  & 139 \\ 
% Adapter  &  12.2  & 42 \\
% FT       & 498.8  & 1 \\
% \bottomrule
% \end{tabular}
% }
% \caption{The size of trainable parameters of PET approaches and fine-tuning. }\label{tab:comm_analysis}
% \end{table}

% \subsection{Baseline}
% \subsection{Experiments Setup}
\subsubsection{Implementation Details} 
We adopt the benchmark FL system FedAvg to simulate the FL setting, which has been applied to commercial products~\cite{bonawitz2019towards}. In FedAvg, clients upload local model parameters to the central server and download the aggregated model for the next training round. Following \citet{lin2021fednlp}, we set the communication round to 100 and the local training epoch to 1 for all tuning methods. Following \citet{chen2022revisiting}, we utilize Roberta-Base~\cite{liu2019roberta} as the local model released by Huggingface\footnote{https://github.com/huggingface/transformers}. The FedAvg implementation is based on \texttt{FedLab}~\cite{zeng2021fedlab}.

Under the FedAvg training protocol, we primarily evaluate the vanilla fine-tuning (FedFT) and four representative PETuning methods, covering adapter (FedAP), prefix-tuning (FedPF), LoRA (FedLR) and BitFit (FedBF). For FedAP, we follow the architecture in \citet{houlsby2019parameter}, which interpose adapter modules into both the multi-head attention module and the feed-forward network in each Transformer layer. We use prefix-tuning~\cite{lester2021power} as the representative of prompt tuning because it has better performance on the small PLMs, e.g., base versions of Roberta.  For LoRA and BitFit, we take the architectures from their origin papers~\cite{zaken2021bitfit,DBLP:conf/iclr/HuSWALWWC22}. All PETuing methods are based on \texttt{OpenDelta} code\footnote{https://github.com/thunlp/OpenDelta}, which is a plug-and-play framework for parameter-efficient-tuning.

To make a fair and reasonable comparison, we run a hyperparameter sweep for each dataset and tuning method. We select the best model according to metric on the validation set and report test-set metric. Specially, the learning rate is selected from \{5e-5, 1e-4, 5e-4, 1e-3, 5e-3, 1e-2\}. We search the reduction factor from \{16, 64\} for FedAP, the prompt length from \{8, 16, 64\} for FedPF, and the scaling factor and rank from \{8, 16\} for FedLR. All experiments are done on a server with 8 Nvidia Tesla V100 GPUs with 32GB RAM each.

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/dlg.pdf}
\caption{} 
\vspace{-0.4cm}
\end{figure}

\subsection{Privacy Results}
The original intention of federal learning is to protect the participants' private data. However, prior work~\cite{zhu2019deep,sun2020provable,boenisch2021curious} has shown how the model updates sent to the server partially reconstruct participants' training data.

% \subsection{Experiment Results}
% To verify the effectiveness of parameter-efficient tuning methods, we conduct a set of experiments comparing four popular PETuning methods to fine-tuning. In this section, our experiments focus on a federated learning setting with FedAvg algorithm [cite] and a centralized setting. 
% \yyh{[del above?]}
% Motivated by the success of PETuning methods in reducing the number of trainable parameters under the centralized setting, we aim to verify the effectiveness of these methods for federated learning to alleviate the communication budget.
% Specifically, we want 

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/comm_exp.pdf}
\caption{Accuracy versus Communication Budget for all tuning methods. The horizontal dashed line indicates the acceptable performance, which is 90\% of the accuracy of FedFT.}
\label{fig:comm_analysis} 
\vspace{-0.4cm}
\end{figure}

\begin{table}[]
\centering
\small
\label{tab:communication_exp}
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|S|S}
\toprule
Methods & RT{E} & MNLI \\
\midrule
BitFit   &  2.6 & 2.6 \\
Prefix   &  41.4 & 41.4 \\
LoRA     &  3.5 & 3.6  \\ 
Adapter  &  4.1  & 11.9  \\
FT       & 498.6 & 498.6 \\
\bottomrule
\end{tabular}
% }
\caption{The size of trainable parameters of PETuning methods and fine-tuning on local clients. }\label{tab:comm_analysis}
\vspace{-0.4cm}
\end{table}

\subsection{Resource Costs Analysis}\label{rq:resouce_cost}
Figure \ref{fig:comm_analysis} shows the communication budget and the accuracy of all tuning methods on RTE and MNLI.\footnote{The plots for the remaining tasks can be found in Appendix \ref{sec:more_comu_analysis}, which have similar results.}  Specifically, we present an acceptable accuracy (90\% of FedFT) with the horizontal dashed line in Figure \ref{fig:comm_analysis}. To achieve desirable performance, all tuning methods in the FL setting need to transmit different sizes of traffic. We find that \textbf{PETuning methods can reduce the communication overhead compared with full fine-tuning by 1\textasciitilde 2 orders of magnitude under the FL setting} when they achieve acceptable performance. As shown in Figure~\ref{fig:comm_analysis}, PETuning methods' communication requirements are ranked as FedPF > FedAP > FedLR > FedBF. Interestingly, the higher communication cost does not indicate a performance gain in PETuning methods. For instance, FedAP consistently outperforms FedPF while having a third of the communication budgets that FedPF needs. We speculate the design of the structure for PETuning may play a greater role. 

% FedLR and FedBF are over 100 times smaller than that of FedFT.
% Among PETuning methods,  FedPF which has the most significant number of communication parameters among PETuning methods can still reduce the cost by over 10 times compared to FedFT. For instance, FedAP consistently outperforms FedPF with a third of the communication budgets that FedPF needs.
% It is also found that PETuning methods have a competitive performance to full fine-tuning.
% For instance, prefix tuning, which has the largest number of tuning parameters among four PETuning methods, lags behind fine-tuning by $5.7\%$ on the RTE task, while adapter tuning achieves a comparable performance to fine-tuning 
% For instance, 

Table \ref{tab:comm_analysis} presents the number of trainable parameters on local clients. We find that \textbf{all PETuning methods can bring efficient local model adaptation cost for clients in FL systems.} These results imply that local devices with limited storage capacity can benefit from PETuning methods since these methods enable sharing a pre-trained model across different tasks and maintaining a few parameters for each task, reducing the storage requirement.
% It is noteworthy that the number of trainable parameters of a method can vary across different tasks due to the different hyper-parameter settings that produce the best performance.


% \textbf{Conclusion:} FedPETuning methods can reduce the communication cost significantly while providing competitive performance to FedFT.



\subsection{Performance Results}\label{rq:acc}
Table \ref{tab:main_results} shows the performance for four PETuning methods and fine-tuning under the federated (upper half table) and centralized settings (bottom half table). This result demonstrates that unlike the success achieved in the centralized setting, \textbf{although PETuning methods are no match for full fine-tuning performance in the federated setting, this performance gap is not insurmountable.}
% For the FL, our default setting is to split the dataset across $100$ clients and sample $10\%$ of clients in each round.

In the centralized setting, PETuning methods achieve competitive performance compared with fine-tuning. Specifically, PETuning methods outperform fine-tuning on five out of six datasets, and the Adapter and LoRA achieve better performances on average. This observation demonstrates tuning all parameters of the pre-trained models is not necessary for achieving the best performance.

% The average performance of Adapter tuning over six tasks is $84.7\%$ and outperforms that of fine-tuning by $1.3\%$. The average performance of fine-tuning over 6 tasks is $83.1\%$. Though FedAP obtains the best performance with $82.4\%$ among four PETuning methods, it lags behind fine-tuning by $0.8\%$.

% Comparing the performance under the centralized setting to that under the federated setting, it is observed that all tuning approaches suffer from a significant drop in performance while fine-tuning is more robust to different settings. More concretely, adapter tuning whiteness a drop by $2.7\%$ while fine-tuning suffers from a drop by $0.6\%$. 
% The most severe degradation is observed by BifFit, of which the performance decreases from $82.6\%$ to $77.8\%$.

However, the observation in the federated setting is quite different from the centralized setting. From the upper half of Table \ref{tab:main_results}, FedFT consistently achieves the best performance on all the datasets since different PETuning methods significantly reduce the local tunable parameters and communication overhead. PETuning methods have different adaptability in federation learning. The performance degradation is drastic for FedBF and FedPF and slight for FedLR and FedAP. The reasons may be that Adapter and LoRA are more robust PETuning methods shown in centralized training and can also work in challenging FL settings.  

Comparing the performance under the centralized setting, we find that all tuning methods suffer from a drop in performance under the federated setting shown in Table~\ref{tab:main_results}. We think it is interesting to design suitable federation learning algorithms combining PETuning methods to bridge the performance gap caused by Non-IID in FL. This will be explored in our future work.

\subsection{Data Scale Analysis}\label{rq:data_scale}
The available data on local clients is slight in real-world FL scenarios such as personal mobile devices. Therefore, it is necessary to explore the performance of federal learning at different data sizes. As shown in Table \ref{tab:benchmark}, different tasks vary in data scale drastically. According to the dataset sizes, we roughly split six tasks into three categories: low-resource datasets (RTE and MRPC), medium-resource datasets (SST-2 and QNLI), and high-resource datasets (QQP and MNLI-mm). 

Considering the data scale into analysis, we find that \textbf{PETuning methods are more unstable compared with FedFT on low-resource datasets.} For instance, the performance of FedLR on RTE and MRPC is over $4.0$ while the standard deviation on other datasets is no more than $0.5$. The apparent difference between performance on low-resource tasks and that on other tasks also holds for other PETuning methods. This phenomenon is consistent with previous work~\cite{chen2022revisiting}, and they show that increasing the training step length can effectively mitigate the instability of the PETuning method. We further explore the effects of local training epochs on PETuning methods under the FL setting.
% On the contrary, FedFT provides a more stable performance over different runs for all datasets.
% we can have the observation that: \textbf{FedTuning are Unstable on Low-Resource Tasks.}

 % Our experimental results in Table \ref{tab:main_results} are reported over five runs with different seeds. The results show that the standard deviation of PETtuning methods is more significant on low-resource tasks than on other datasets under centralized and federated settings. For instance, the performance of FedLR or LoRA on RTE and MRPC is over $4.0$ while the standard deviation on other datasets is no more than $0.5$. The apparent difference between performance on low-resource tasks and that on other tasks also holds for other PETuning methods.

% Compared to PETuning methods, FedFT provides more stable performance over different runs.
% Specifically, FedFT obtains the smallest deviation on four out of six tasks.
% Since local clients have access to only a portion of training data,
% The severe data scarcity under the federated setting reveals that PETuning methods fall short of handling tasks with few training samples.
% Despite the advantage of FedFT over PETuning methods, fine-tuning in the centralized setting has no advantage over PETuning methods.

% \textbf{Federated Setting is Sensitive to Low-Resource Tasks. \yyh{[need paraphrase]}}
% Comparing the performance under the federated setting to that under the centralized setting, we found that average performance over tuning methods on low-resource tasks suffers from a more serious drop.
% Specifically, the RTE and MRPC tasks witness a drop in performance by $9.2\%$ and $4.3\%$ by switching to the federated setting, respectively.
% On the contrary, the average performance on SST-2 decreased by only $0.4\%$.
% This observation demonstrates that the data scale is a crucial factor that influences the effectiveness of tuning methods under the federated setting.

% PETuning methods perform stably on large-scale datasets. From Tabel \ref{fig:sample}, it is observed that the performance of PETuning methods changes drastically with varying the sample ratio on the low-resource and medium-resource tasks. 
% For instance, on CoLA,  prefix tuning suffers from a drop in performance over 10\% by changing the sample ratio from 0.1 to 0.3. A consistent drop in performance of prefix tuning is also observed on SST-2.
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/epoch_exp.pdf}
\caption{Accuracy comparison of PETuning methods and FT under different epochs.}
% The performance of PETuning approaches on \fedglue with different numbers of training epochs.} 
\label{fig:epoch} 
% \vspace{-0.4cm}
\end{figure}

% \subsection{Impact of Local Epochs}\label{rq:epoches}
% Figure \ref{fig:epoch} shows the accuracy of PETuning methods and FT with different numbers of local training epochs. we can find that the impact of the number of local training epochs varies with the scale of datasets.
% Specifically, clients trained with more epochs consistently yield a performance gain across different tuning methods for tasks with abundant training samples. For instance, on MNLI, all the tuning approaches obtain an improvement in performance with the number of epochs as 2 and 3.
% More examples are provided in Appendix \ref{sec:more_epoch_analysis}.

% For tasks with fewer samples, training with more epochs can incur a drop in performance. Take RTE as an example. Four out of five tuning methods suffer from performance degradation with the number of local training epochs as 3.
% Though an improvement in performance can be witnessed in several settings, the magnitude of performance degradation is more significant than the improvement.
% We further explore the relative accuracy with different numbers of local training epochs.
% In Figure \ref{fig:epoch}, 

Figure \ref{fig:epoch} shows the accuracy of PETuning methods and FT with different numbers of local training epochs on RTE and MNLI. More results are provided in Appendix \ref{sec:more_epoch_analysis}. This result reveals that \textbf{for all PETuning methods and FT, the local data scale under the FL setting also influences the effect of increasing the number of training epochs.}  Specifically, clients trained with more epochs in the FL system consistently yield a performance gain across different tuning methods for datasets with large training samples (like MNLI). In comparison, training with more epochs can incur a drop in performance for the low-resource dataset (like RTE) in most cases. The reason may be that increasing the number of training epochs for FL clients with small data samples makes PLMs more prone to overfitting. However, datasets with high resources require more local training epochs to improve the performance of FL.



\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/relative_alpha_exp.pdf}
\caption{Relative performance of PETuning methods on \fedglue under different Dirichlet distributions.} 
\label{fig:alpha} 
\vspace{0.3cm}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/distribution_exp.pdf}
\caption{Data distribution under different $\alpha$. We report the pairwise Jensen–Shannon distance of the label distribution between two clients.}
\label{fig:distribution} 
\vspace{-0.4cm}
\end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.48\textwidth]{images/sample_exp.pdf}
% \caption{The performance of FedPETuning on \fedglue with different sample ratios.} 
% \label{fig:sample} 
% \vspace{-0.4cm}
% \end{figure}


% In application scenarios, the setting of federated learning can vary drastically. 
% Having shown that PETuning methods are competitive alternatives to full fine-tuning in our standard setting, it is critical to verify the capability of PETuning methods to maintain high performance in other settings.
% In this section, we study the PETuning methods under different federated learning settings by varying data distribution, federated scenarios, and training settings.
% the alpha $\alpha$ that indicates the extent of non-IID, and the sample ratio which reflects the participation tensity of clients.

\subsection{Impact of Data Distribution}\label{rq:alpha}
We turn to \textbf{RQ4} in this section. Figure~\ref{fig:alpha} illustrates the performance of PETuning methods and FT under different data distributions. In this experiment, we consider three Dirichlet distributions by choosing $\alpha$ from $\{0.1, 1.0, 10.0\}$ where a smaller $\alpha$ indicates a sharper non-IID distribution. 

As shown in Figure~\ref{fig:alpha}, the data distribution heterogeneity significantly impacts all tuning methods' performance. In most cases, increasing data heterogeneity leads to performance degradation for all tuning methods on different datasets. \textbf{Compared to FedFT, PETuning methods are more susceptible to data heterogeneity in the FL setting.} The evidence is that the performance of PETuning methods degrades more drastically when the data heterogeneity increases, as in the case of MNLI and RTE. This result shows although PETuning significantly reduces communication, the data distribution shift impacts the federated aggregation of uploaded lightweight parameters. Other tasks' results can be found in Appendix \ref{sec:more_alpha_analysis}.

% As  can be seen, varying data distributions can significantly impact the model performance.
% Increasing alpha from $0.1$ to $1.0$ consistently leads to better performance for all tuning methods on different tasks, except for the FedLR on RTE. 
% % Since a smaller alpha indicates a sharper non-IID scenario, 
% This observation indicates that all the approaches can be influenced by the  distribution shift issue and prefer an IID setting.

% When increasing the alpha from $1.0$ to $10.0$, an expected improvement is also observed in almost all settings. 
% % For example, on the RTE task, the performance of LoRA decreases from over $65.0$ to performance worse than $60.0$ while BitFit method suffers from degradation of about $2$ points on MRPC. 
% However, a slight decrease in performance can be found with FedAP on the RTE task.
% A more apparent drop is observed on MRPC with FedBF that the performance with $\alpha$ as $10.0$ is as worse as the performance when $\alpha$ equals $0.1$,
% as shown in Appendix \ref{sec:more_alpha_analysis}.
% Since tasks considered in our experiments have no more than three categories, we hypothesize that increasing $\alpha$ from $1.0$ to $10.0$ can have little impact on label distributions, as shown in Figure \ref{fig:distribution}.

When increasing the alpha from $1.0$ to $10.0$, we find that the performance of all tuning methods does not change much. The data heterogeneity, which did not change significantly, contributed to the result. Figure~\ref{fig:distribution} reports the Probability Density Function (PDF) of the data distribution under different $\alpha$. The data heterogeneity is similar for $\alpha$ equal to 1.0 and 10.0, while the distribution gap is large for $\alpha$ equal to 0.1. 


\subsection{Various FL scenarios}\label{rq:fl_scen}
% The client status in FL is determined by the number of total clients and the percentage of clients that participate in each round. 
% To verify the effectiveness and robustness of PETuning methods under various settings, we conduct a set of experiments by varying the sample ratio that determines the availability ratio of clients in each round, and the number of total clients, respectively.

% The total number of clients and the ratio of clients that participate in each communication round are two important factors that determine federated scenarios.
To verify the effectiveness of PETuning methods under different FL scenarios, we mainly consider two standard settings in this section: the cross-silo setting~\cite{kairouz2021advances} and the large-scale setting~\cite{lai2022fedscale}. In this experiment, we chose RTE, MRPC, and SST-2 to simulate the cross-silo setting, while QNLI, QQP, and MNLI to simulate the large-scale setting. The total number of clients in the cross-silo and large-scale settings is 10 and 1000, respectively. And ten clients are involved in each communication round for local training and federated aggregation. 

Table~\ref{tab:cross-silo} and Table~\ref{tab:large-scale} show the performance results of PETuning and FT under these two FL scenarios, respectively. The results show that \textbf{PETuning methods can also significantly reduce the communication overhead while achieving acceptable performance in cross-silo and large-scale settings.} More noteworthy between the different FL scenes is the cross-silo setting. As shown in Table~\ref{tab:cross-silo}, the cross-silo setting diminishes the performance gap between the PETuning methods and fine-tuning, compared to our standard setting in Section~\ref{rq:acc}. For example, FedPF lags behind FedFT by $2.7\%$ and $6.5\%$ under the cross-silo and standard settings, respectively. We attribute this observation to relieving the data scarcity issue since each client has ten times more training samples in the cross-silo setting than in the standard setting.

% \textbf{Cross-silo.} 
% Table \ref{tab:cross-silo} shows the experimental results on three tasks with the number of clients as 10 and the ratio of participated clients as 1.0.
% Considering the number of training samples held by each client is in inverse proportion to the number of total clients, we use the tasks with a relatively small data scale for the cross-silo setting.

% \textbf{Large-scale.} 
% Table \ref{tab:cross-silo} shows the experimental results on the remaining three tasks with the total number of  clients as 1000.
% For a fair comparison, the sample ratio is set as 0.01.
% It is observed that FedFT outperforms all PETuning methods due to the severe data scarcity brought by the large number of clients.

% \textbf{Sample Ratio.}
% We compare tuning methods over the sample ratio from $\{0.1, 0.2, 9.3, 0.4\}$ on six tasks.
% As shown in Figure \ref{fig:sample},
% it is observed that the performance of most of the tuning approaches varies slightly on high-resource tasks with different sample ratios. For instance, there is no approach whose performance varies by over $1\%$ on the QQP task. 
% Drastic fluctuations in performance over different sample ratios are observed on RTE.
% For instance, both FedLR and FedPF suffer from a drop in performance by $5\%$ as sample ratio increases from $0.3$ to $0.4$.

\begin{table}[t]
    \centering
    
    % \scalebox{0.98}{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccc|lrl}
    \toprule
    Methods & RTE & MRPC & SST-2 & Avg. & \multicolumn{1}{c}{Rel.} & Com. \\
    \midrule
    FedFT  & $70.4$ & $90.2$ & $94.3$ & $85.0$ & $100.0$\% & $1$x\\
    FedAP & $71.5$ & $88.5$ & $94.0$ & $84.7$ &
    \yblue{$99.7\%$} & \ygreen{$\uparrow$}$70$x \\
    FedLR & $70.8$ & $89.8$ & $94.4$ & $85.0$ &
    \yred{$100.0\%$} & \ygreen{$\uparrow$}$141$x \\
    FedPF & $66.4$ & $88.1$ & $93.7$ & $82.7$ &
    \yblue{$97.3\%$} & \ygreen{$\uparrow$}$12$x \\
    FedBF &  $55.2$ & $88.6$ & $92.8$ & $78.9$ & 
    $92.8\%$ & \ygreen{$\uparrow$}$189$x \\

    \bottomrule
    \end{tabular}
    }
    \caption{Performance results of the PETuning methods and FT in the cross-silo setting. In this setting, we set the total number of clients in the FL system as 10 and the client sample ratio as 1.0.}  \label{tab:cross-silo}
\end{table}


\begin{table}[t]
    \centering
    
    % \scalebox{0.98}{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccc|lrl}
    \toprule
    Methods & QNLI & QQP & MNLI & Avg. & \multicolumn{1}{c}{Rel.} & Com. \\
    \midrule
    FedFT & $87.9$ & $88.8$ & $85.6$ & $87.4$ & $100.0$\% & $1$x\\
    FedAP & $85.9$ & $87.0$ & $84.9$ & $85.9$ &
    \yblue{$98.3\%$} & \ygreen{$\uparrow$}$52$x \\
    FedLR & $86.0$ &  $86.5$ & $84.7$ & $85.7$ &
    \yblue{$98.1\%$} & \ygreen{$\uparrow$}$140$x \\
    FedPF & $84.6$ & $81.8$ & $80.4$ & $82.3$ &
    $94.2\%$ & \ygreen{$\uparrow$}$12$x \\
    FedBF & $80.5$ & $84.0$ & $80.7$ & $81.7$ &
    $93.5\%$ & \ygreen{$\uparrow$}$190$x \\
    \bottomrule
    \end{tabular}
    }
    \caption{Performance results of the PETuning methods and FT in the large-scale setting. In this setting, we set the total number of clients in the FL system as 1000 and the client sample ratio as 0.01.}  \label{tab:large-scale}
\end{table}

==> background.tex <==
We start by introducing the background of FL and PETuning methods. Then, we elaborate on the necessity of introducing PETuning methods into federated training process, which are the fundamental motivation of our work.

% benchmarking PLMs tuning methods in FL settings as well as

\paragraph{Federated Learning.} Recently, federated learning~\cite{mcmahan2017communication} (FL) has emerged as a privacy-preserving technique designed to collaboratively train deep learning (DL) models without sharing or uploading the client data from personal customers, small businesses, and large enterprises to a centralized, third-party server. Instead, the client computes and sends model gradients to a server, which aggregates them to produce a global model. As the client data remains on the local device, FL has widely been applied to privacy-sensitive NLP tasks~\cite{liu2021federated,ge2020fedner,sui2020feded}.

\paragraph{Parameter-efficient Tuning.} In the era of large-scale pre-trained language models (PLMs), PLMs bring the blessing of effectiveness to NLP applications while posing prohibitive model adaptation cost challenges~\cite{ding2022delta}. Recently, a large body of work has developed various parameter-efficient tuning (PETuning) methods designed to utilize lightweight tunable parameters to "evoke" colossal PLMs~\cite{li-liang-2021-prefix, DBLP:journals/corr/abs-2110-07602, houlsby2019parameter, DBLP:conf/iclr/HuSWALWWC22, zaken2021bitfit}. In PETuning methods, most parameters of PLMs keep frozen and only a few additional parameters or a fraction of the PLMs' parameters are optimized for downstream tasks. As such, PETuning methods dramatically reduce model adaptation's computational cost, storage requirement, and task-switching overhead. 

% \paragraph{Needs for PLMs tuning Benchmark in FL setting.} 

\paragraph{Communication Constraints.} Communication cost is an open problem in FL, primarily due to model updates high-frequently exchanged between clients and the server~\cite{zhao2022towards}. With PLMs becoming the preferred backbone for downstream tasks, tremendous communication overhead caused by large-scale PLMs' updates undoubtedly poses a more critical challenge for applying FL to NLP tasks~\cite{passban2022training}. Tuning PLMs in FL way takes excessive time during frequent upload-download processes, making it intolerably slow and impractical in real scenarios~\cite{sui2020feded}. Therefore, developing a communication-efficient method that suits PLMs' federated tuning is necessary. In general, FL mainly communicates entire model updates between clients and the server. In this sense, PETuning methods with light-weight trainable parameters could be a promising technique for tuning PLMs in the FL setting, as opposed to updating and sending the entire PLMs.


